PowerNorm: Rethinking Batch Normalization in Transformers

The standard normalization method for neural network (NN) models used in Natural Language Processing (NLP) is layer normalization (LN). This is different than batch normalization (BN), which is widely-adopted in Computer Vision. The preferred use of LN in NLP is principally due to the empirical observation that a (naive/vanilla) use of BN leads to significant performance degradation for NLP tasks; however, a thorough understanding of the underlying reasons for this is not always evident. In this paper, we perform a systematic study of NLP transformer models to understand why BN has a poor performance, as compared to LN. We find that the statistics of NLP data across the batch dimension exhibit large fluctuations throughout training. This results in instability, if BN is naively implemented. To address this, we propose Power Normalization (PN), a novel normalization scheme that resolves this issue by (i) relaxing zero-mean normalization in BN, (ii) incorporating a running quadratic mean instead of per batch statistics to stabilize fluctuations, and (iii) using an approximate backpropagation for incorporating the running statistics in the forward pass. We show theoretically, under mild assumptions, that PN leads to a smaller Lipschitz constant for the loss, compared with BN. Furthermore, we prove that the approximate backpropagation scheme leads to bounded gradients. We extensively test PN for transformers on a range of NLP tasks, and we show that it significantly outperforms both LN and BN. In particular, PN outperforms LN by 0.4/0.6 BLEU on IWSLT14/WMT14 and 5.6/3.0 PPL on PTB/WikiText-103. We make our code publicly available at \url{https://github.com/sIncerass/powernorm}.

==> algo.tex <==
% \begin{algorithm}[]
%     \caption{Adaptive Batch Size }
%     \label{alg:abs}
%     \begin{algorithmic}[1]
%         \STATE {\bf Input:} 
%         \begin{compactitem}[\bfseries -]
%             \item Learning rate $lr$, learning rate decay steps $A$, learning rate decay ratio $\rho$
%             \item Initial Batch Size $B$, minimum batch size $B_{min}$, maximum batch size $B_{max}$, input $x$, label $y$.
%             \item Eigenvalue decreasing ratio $\alpha$, eigenvalue computation frequency $n$, i.e.,  after training $n$ samples compute eigenvalue, batch increasing ratio $\beta$, duration factor $\kappa$, i.e.,  if we compute $\kappa$ times Hessian but eigenvalue does not decrease, we would increase the batch size
%             \item If adversarial training is used, perturbation magnitude $\epsilon_{adv}$, perturbation ratio $\gamma$ ($\gamma_{max}$) of training data, decay ratio $\omega$, vanishing step $\tau$
%         \end{compactitem}    
%         \STATE {\bf{Initialization:} Eig = None, Visiting Sample = 0}
%         \FOR{$ t = 0,1,\ldots $}
%         \IF{$\gamma>0$}
%         \STATE $x[:B*\gamma] = adversarial(x[:B*\gamma])$
%         \ENDIF
%         \STATE One step SGD updates
%         \STATE Visiting Sample = Visiting Sample + B
%         \IF {Visiting Sample \% n is $0$}
%             \STATE Current Eigen = Computing Eigenvalue
%             \IF {itr Eigen $<$ $\frac12*$Eig}
%             \STATE $B=\min{B*\beta, B_{max}}$, increasing the learning rate proportional to batch size changing
%             \STATE $\gamma=\gamma/2$, Eig = Current Eigen
%             \STATE Duration Time = 0 
%             \ELSE 
%             \STATE Duration Time = Duration Time $+$ 1
%             \ENDIF
%         \ENDIF
%         \IF{Duration Time = $\kappa$}
%         \STATE $B=\min{B*\beta, B_{max}}$, increasing the learning rate proportional to batch size changing
%         \STATE Duration Time = 0 
%         \ENDIF
%         \IF{t in A}
%         \STATE decay the learning rate by $\rho$
%         \ENDIF
%         \IF{$t==\tau$}
%         \STATE $\gamma=0$
%         \ENDIF
%         \ENDFOR
%     \end{algorithmic}
% \end{algorithm}

\begin{algorithm}
\DontPrintSemicolon
\caption{Adaptive Batch Size (ABS) and Adaptive Batch Size Adversarial (ABSA)}\label{alg:abs}
% \begin{algorithmic}[1]
        % \State {{\footnotesize\bf Input:}}
        % % \algorithmicinput
        % \begin{compactitem}[\bfseries -]
        % {\footnotesize%\scriptsize%
        %     \item Learning rate $lr$, learning rate decay steps $A$, learning rate decay ratio $\rho$
        %     \item Initial Batch Size $B$, minimum batch size $B_{min}$, maximum batch size $B_{max}$, input $x$, label $y$.
        %     \item Eigenvalue decreasing ratio $\alpha$, eigenvalue computation frequency $n$ (i.e.,  after training $n$ samples compute eigenvalue), batch increasing ratio $\beta$, duration factor $\kappa$ (i.e.,  if we compute $\kappa$ times Hessian but eigenvalue does not decrease, we would increase the batch size)
        %     \item If adversarial training is used, perturbation magnitude $\epsilon_{adv}$, perturbation ratio $\gamma$ ($\gamma_{max}$) of training data, decay ratio $\omega$, vanishing step $\tau$}
        % \end{compactitem}    
        % \State {{\footnotesize\bf{Initialization:} Eig = None, Visiting Sample = 0}}
        % \For{{\footnotesize$ t = 0,1,\ldots $}}
        % \If{{\footnotesize$\gamma>0$}}
        % \State {\footnotesize $x[:B\gamma] = adversarial(x[:B\gamma])$}
        % \EndIf
        % \State {\footnotesize One step SGD updates}
        % \State {\footnotesize Visiting Sample $+=$ B}
        % \If {{\footnotesize Visiting Sample \% n is $0$}}
        %     \State {\footnotesize Current Eigen = Computing Eigen}
        %     \If {{\footnotesize Current Eigen $<$ $\frac12*$Eig}}
        %     \State {\footnotesize $B=\min\{B\beta, B_{max}\}$, change $lr$ proportional to batch size changing}%increasing the learning rate proportional to batch size changing
        %     \State {\footnotesize$\gamma=\gamma/2$, Eig = Current Eigen}
        %     \State {\footnotesize Duration Time = 0 }
        %     \Else
        %     \State {\footnotesize Duration Time $+=$  1}
        %     \EndIf
        % \EndIf
        % \If{{\footnotesize Duration Time = $\kappa$}}
        % \State {\footnotesize$B=\min\{B\beta, B_{max}\}$, change $lr$ proportional to batch size changing} %increasing the learning rate proportional to batch size changing
        % \State {\footnotesize Duration Time = 0 }
        % \EndIf
        % \If{{\footnotesize t in A}}
        % \State {\footnotesize decay the learning rate by $\rho$}
        % \EndIf
        % \If{{\footnotesize $t==\tau$}}
        % \State {\footnotesize$\gamma=0$}
        % \EndIf
        % \EndFor
    % \IF{some condition is true}
    %     \STATE do some processing
    % \ELSIF{some other condition is true}
    %     \STATE do some different processing
    % \ELSE
    %     \STATE do the default actions
    % \ENDIF        
% \end{algorithmic}
   \SetAlgoLined
    \KwInput{Learning rate $\eta$, decay epoch $E_{decay}$, decay ratio $\rho_{lr, decay}$; initial batch $B_{init}$, maximum batch $B_{max}$; Eigenvalue decay ratio $\alpha$, batch/lr increasing ratio $\beta$, duration factor $\kappa$; adversarial input ratio $\gamma$, adversarial magnitude $\epsilon_{adv}$, adversarial input ratio decay factor $\omega$, terminate epoch $\tau$; input data $x$. }
    \KwResult{Final model parameters $\theta$}
    Initialize old (new) eigenvalue as $\lambda_{old}$ ($\lambda_{new}$), batch size $B_{itr}$, learning rate $\eta_{itr}$, duration time $\kappa_{itr}=0$.
    
    \For{Epoch $=1,2,3\ldots$}{
      \For(\tcp*[h]{mini-batch iterations}){$t=1,2,3\ldots$}{
        generate adversarial data $x_{adv}$ by the ratio of $\gamma$;
        
        SGD update;
      }
     
      compute $\lambda_{new}$; \tcp*[h]{Hessian power-iteration}
      
      $\kappa_{itr} \pluseq 1$;
      
      $Flag = \{(\lambda_{new} < \lambda_{old}/\alpha)~OR~(\kappa_{itr}=\kappa)\}$;
       
      \If(\tcp*[h]{adaptively change batch/lr}){Flag}{
      $B_{itr}\asteq\beta$;~~
      $\eta_{itr}\asteq\beta$;
      $\gamma \diveq \omega$;~
      $\kappa_{itr}=0$;~
      }
      \If{$\lambda_{new} < \lambda_{old}/\alpha$}{
      $\lambda_{old}=\lambda_{new}$;
      }
      
      \If{Epoch $=\tau$ }{
        $\gamma = 0$;
      }
      \If(\tcp*[h]{lr decay schedule}){Epoch in $E_{decay}$}{
      $\eta_{itr} \diveq \rho_{lr, decay}$ ;
      }    
    }
\end{algorithm}





==> makefile <==
compilePdfOptions=
compPdftex=pdflatex ${compilePdfOptions}
compile= ${compPdftex}

TARGET=bin/main.pdf
#TARGET= bin/sigconf.pdf
MAIN=main.tex
FILES=main.tex


.SECONDEXPANSION:

####################  COMPILE PDF  ######################

all: ${TARGET}

bin/%.pdf : ${FILES} # .figs_ 
	mkdir -p bin
	#latexmk  -pvc -bibtex -pdf ${MAIN}
	${compile}  $*
	-bibtex $*
	-bibtex $*
	${compile} $*
	${compile} $*
	#${compile} $*
	mv $*.pdf $@
	#make clean
	#open ${TARGET}
	@echo Done ....!


##############  EXTERNALIZE TIKZ-FIGURES  ###############

# TIKZ_FIGS_DIR=tikz_figs
# FIGS=$(shell grep -h '[:space:]*\\inputtikz' ${TIKZ_FIGS_DIR}/figures.tex | sed '1D' | \
#   sed s'/[:space:]*\\inputtikz{\(.*\)}{/\1/' )
# FIGSPDF=$(FIGS:%=%.pdf)
# 
# .figs_ : $(FIGSPDF)
# 	date &> .figs_
# 
# ${TIKZ_FIGS_DIR}/%.pdf : $$(word 1, $$(subst -, ,$${TIKZ_FIGS_DIR}/%)).tex
# 	${compile} --jobname=${TIKZ_FIGS_DIR}/$* \
# 	  '\newcommand{\fakejobname}{${TIKZ_FIGS_DIR}/$*}\input{${TIKZ_FIGS_DIR}/figures.tex}'
# 
########################  CLEAN  ########################

cleanall: clean
	rm -r -f bin/*.pdf ${TIKZ_FIGS_DIR}/*.pdf .figs_
	cd      figs/matlab && ./clean.sh
	cd tikz_figs/matlab && ./clean.sh
	@echo Cleaned All ....! 

clean:
	rm -f *.aux *.dvi *.blg *.out *.log */*.log */*/*.log *~ */*~ *.fdb_latexmk *.fls *.xml* *.out
	@echo Cleaned ....! 


